Improving Deep Learning with Differential Privacy using Gradient Encoding and Denoising

Deep learning models leak significant amounts of information about their training datasets. Previous work has investigated training models with differential privacy (DP) guarantees through adding DP noise to the gradients. However, such solutions (specifically, DPSGD), result in large degradations in the accuracy of the trained models. In this paper, we aim at training deep learning models with DP guarantees while preserving model accuracy much better than previous works. Our key technique is to encode gradients to map them to a smaller vector space, therefore enabling us to obtain DP guarantees for different noise distributions. This allows us to investigate and choose noise distributions that best preserve model accuracy for a target privacy budget. We also take advantage of the post-processing property of differential privacy by introducing the idea of denoising, which further improves the utility of the trained models without degrading their DP guarantees. We show that our mechanism outperforms the state-of-the-art DPSGD; for instance, for the same model accuracy of $96.1\%$ on MNIST, our technique results in a privacy bound of $\epsilon=3.2$ compared to $\epsilon=6$ of DPSGD, which is a significant improvement.

==> algorithms/distretization_alg.tex <==
\begin{algorithm}[t!]
	\caption{Gradient Discretization}
    \begin{algorithmic}[1]
        \STATE $\tau \gets$ threshold
        \STATE $\nabla \gets$ parameters' gradient
        \FORALL{ $v$ in $\nabla$}  
        \IF {$v > \tau $}
        \STATE $ v = 1$ \COMMENT{UP}
        \ELSIF{{$v < -\tau $}}
        \STATE $ v = -1$ \COMMENT{DOWN}
        \ELSE
        \STATE $ v = 0$ \COMMENT{STOP}
        \ENDIF
        \ENDFOR
        \RETURN $\nabla$
	\end{algorithmic}
	\label{alg:discretization}                       
\end{algorithm}



==> algorithms/mainalgorithm.tex <==
\begin{algorithm}[t!]
	\caption{Differentially Private Discrete SGD}
    \begin{algorithmic}[1]
	\REQUIRE learning rate $\eta$, $\mu$-batchsize $\mu$, batchsize $n$, noise scale $\sigma$, gradient threshold $\tau$, gradient norm clip $C$
	\STATE Initiate $\theta$ randomly
	\FOR{$t \in \{T\}$}
	\STATE $B_t \gets$ Sample $n$ instances from dataset randomly
	\STATE $\nabla_\theta^G \gets \vec{0}$ 
	\FORALL{$ \mu$-batch  $\in B_t$}
	\STATE Compute gradient of micro-batch $\nabla_\theta^{\mu}$
	\STATE $\nabla_\theta^{\mu} \gets $Discretize gradients using Algorithm~\ref{alg:discretization} given $\tau$ and $\nabla_\theta^{\mu}$
	\STATE Clip gradient $\widetilde{\nabla_\theta^{\mu}} \gets \nabla_\theta^{\mu}\times C / 	max(C,||\nabla_\theta^{\mu}||_2) $
	\STATE $\nabla_\theta^G \gets \nabla_\theta^G  + \widetilde{\nabla_\theta^{\mu} }$
	\ENDFOR
	\STATE $\widetilde{\nabla_\theta^G} \gets \nabla_\theta^G  + \mathcal{N}(0,\sigma^2C^2\mathbb{I})   $
	\STATE $\widehat{\nabla_\theta^G} \gets$Error correction on $\widetilde{\nabla_\theta^G}$
	\STATE $\theta \gets \theta  - \eta \widehat{\nabla_\theta^G}$
	\ENDFOR
	\RETURN output $\theta$ and privacy cost
	\end{algorithmic}
	\label{alg:main_alg}                       
\end{algorithm}



==> algorithms/noise_correction.tex <==
\begin{algorithm}[t!]
	\caption{Independent  Noise Correction}
    \begin{algorithmic}[1]
    	\REQUIRE Private gradients $\widetilde{\nabla_\theta^G}$, batch treshold $\nu$, noise scale $\sigma$, gradient norm clip $C$
        \FORALL{ $v$ in $\widetilde{\nabla_\theta^G}$}  
		\IF{$\Pr(H_U|v,C,\sigma) > \Pr(H_D|v,C,\sigma)$ and $\Pr(H_S|v,C,\sigma) $}
		\STATE $v  = \nu$
		\ELSIF{$\Pr(H_D|v,C,\sigma) > \Pr(H_U|v,C,\sigma)$ and $\Pr(H_S|v,C,\sigma) $}
		\STATE $v  = -\nu$
		\ELSE
		\STATE $v = 0$
		\ENDIF
        \ENDFOR
        \RETURN corrected gradients 
	\end{algorithmic}
	\label{alg:noise_correction}                       
\end{algorithm}



==> code/.git/objects/09/2bcd15a32898499a521ec2f9b4b96771386d54 <==
xTM‹Û0íY¿bHJ xIÃnӅúuÙÓ²E7"²¤ê#iXö¿W²o¼Í¡¾ϼ½÷fä­2[X­>¬ÞµÎtà1DŒQdgCd	­Ô¢±ŒïÙ/ô¤Çãø®ŠA*_qküP{iô¹ôc"Jܟ£KØ<|ºk>ÿøvÿŸõkßTŸ"¼‡/˜>g— 5WQ "ÂæçÐe*¤3"*ôPÃ#ô\öœÓ^'G–"ø$Eé²Gfôø<RïøMJÞ\¢›hŽŽY‹.[@ŸKòÔskA8遘Tl«I&Ä@0£]D¶¯Ö¬û³ë*wÖb>òÉŽ\¥»Æ¿RD$È)2'qŀÁ‰Á…ë
öè4ªŠÇäBOxAH@|ãðw"ÇP{ʉij÷ê»9'u†#&wÌ°p¤_ÄA¸fÖÿŽªÈ,ƒ®éªZ•@ϝ´!Í¿¦w©áë|ój*ìP–ÓЉMÞäR¼ÇÓÑ8ákzYW',†q©©Fj"¯2†}ô"lƒ]xMـ©Ô€¹•ÚIVµ®€Ïw©žÜ¬ùq‡.©MÛFÓ.e×°ÒÕϳÙf)9{'i‰š²,uy‰‰óõäk¬tlœMý<îíg³†+5åPÞ	®˜÷—EÛ|×ó/€®azïûÆ/dAþß&nQ

==> code/.git/objects/68/b99395261c987a070807e19df80bf84815182a <==
xU'Ánƒ0†wæ),.‰U¦]*ñ
}jBL‰'(	0Þ~NÂVÆ!$öï?ŸVê>Þ//b2ÚzPód6@ÊdYÖӐ"#´ÝèXB}WNŸUÖâVÁòÿèDOõIÒàOå5þò<¿E߅¬Zàh~D«¶_ZôÝøº
GÀB³yÍ÷''Åw»_·øWV¯®A¨ÏnDC÷ËgL)³T :-]³"¬Y'æP©gÏñ	¿w=²>Z.eT¥<7J"ñ[±«8úô­ ÷›¡šER«GªCs$‹=[²ã>…0	K~¶
BŠiAqû‡u
o@'›.N-
Ú'
,ª=aæŒvÜ\ž¦Šp<œ@ƇðZaIð; [e?ðc®ô

==> code/.git/objects/b2/67c4f93a6324caec40d34bda4534f79f55d9d2 <==
x­TMoÛ0ÝY¿'èÅàî†a@'î\ìÒ\º!Pl:jˆ$͂ü÷Q¢9i»`9DÅ''ÚÔí®?çù;Ýt­õàuƒÚ1n[[<ŽÓ7Ý"Ӊʶ
øpêP…c	ljË âÖS›Kðiç¹XÐ×GZW´^Ó*,v¨¼£í‡\vƒv<ê¬6>@¿*Y¢)eŸ`zõM'
çïAÁÃay"g8,Žß'öÝɾ:³Sd*C›-TÊytL´†¤Ž`{ã&W¡*ƒ
ð‹ž0gÉÀó?F^GœÃN&ßÌpš2ìh/fBˆ+Ø¢_+kÕÞ¥³›X"L7,§´Zeʶ‰‹I—,f¨gíäõ,ºïØýÒmŧmïù›Îï×µ~Ât—Aé÷Jº½n͖=-úÞPÐ9Á&ùy4"KKÜé'iFQp¦ü²à,)Fô–ˆöº¡œò林/0«KLtä
Ø5H¸t+b·_E銅;/úR͵[«ÒµÚÔ8²ôŨèâö$4Ûýƒ<bü—¼"¶Me¸ž€ÊTe»Œr–w­ÁÌéeRc品6.g
љcþMB±E<¦rå9+—‡ÆùÆË«—óHáB‡§™]ñ9R@'¯N
 áLÕ9xméQµ"ÚÎÌ¡å0;lぐ¼ây¤"»ð¶Ü@'A£M3$Mó¤OB]O±ùyz¥¦ò½þKI炖	Lfÿ­¾Û¯÷§êèæóÚþ¬Èí[Õ©rW§\ªïwtÄ^ïòJh`NœÜ}G¯õ>ØÏû,,ïA·÷_'¢¨ê3¢~'4|

==> code/.git/objects/c1/1372ec01992cdbe16656080c880ddb81305c7d <==
xu']kÂ0†w_q¨0,ìB¯ºZfÙlŦ°]…´3P[iRçþ÷¥:ñ£xyN'çyÉ9iQ¥ð<|zèÉ2+š\€¥¯³•ªj-r–59gß5ßlDí¬,"ðú}¥õ'g¡^.–²àM}ïyÉÄÅ;.enû:Ã;Gÿl&ŽT&6ôv`ÁºQRÚW Ei¬¹%F!
^"(‰;ÜX•Z~5U£:ØóQ‡"󄶸«ÐãSyiDh[Éîþ
æz4¢‡èÀm¸¨¶WU-"
iU d.X!–š _ÿÎc"NÆ7m§c@¦g®u"aã7҃é,£=Bóϗ œ‡lM'wÓháM™ÿAý0¢…îÌ·aM M´vÌHñýE°lxìÈO[b_oàv¶Ä2'÷èç'ď

==> final_alg.tex <==
\section{Experimental Details}

\begin{algorithm}[h!]
%  \scriptsize
     \caption{Differentially Private Discrete SGD}
    \begin{algorithmic}[1]
    \Require{ learning rate $\eta$, $\mu$-batchsize $\mu$, batchsize $n$, noise models $\mathcal{Z}=\{Z_1,Z_2,\cdots,Z_T\}$, preselected gradient vectors $\Psi$}
    \State Initiate $\theta$ randomly
    \For{$t \in \{T\}$} 
    \State $B_t \gets$ Sample $n$ instances from dataset randomly 
    \State $\nabla_\theta^G \gets \vec{0}$ 
    \For{$\mu$-batch $b$  $\in B_t$}
    \State  $\nabla_\theta^{\mu} \gets$ gradient of micro-batch     $b$
    \State $\widecheck{\nabla_\theta^{\mu}} \gets $ encode gradients by solving equation \eqref{eq:select} 
    \Comment{Encoding}
    \State $\nabla_\theta^G \gets \nabla_\theta^G  + \widecheck{\nabla_\theta^{\mu} }$ 
    \EndFor
    \State $\mathcal{Z} \sim Z_t $
    \State $\widetilde{\nabla_\theta^G} \gets \nabla_\theta^G  + \mathcal{Z}$ \red{Noise Addition}
    \State $\widehat{\nabla_\theta^G} \gets$Error correction on $\widetilde{\nabla_\theta^G}$ \red{Error Correction}
    \If{$\text{KS}(\widehat{\nabla_\theta^G},Z_t) > \tau$}
	    \State $\theta \gets \theta  -   \text{KS}(\widehat{\nabla_\theta^G},Z_t) \eta \widehat{\nabla_\theta^G}$
	\EndIf
    \EndFor
    \Return output $\theta$ and privacy cost
    \end{algorithmic}
                    
\end{algorithm}


==> implementation.tex <==
\section{Implementation Details} 
In Section~\ref{}, we described main components of our framework. Training a deep neural network is a time and memory consuming task, unfortunately different components in our framework will increase training time significantly and make them infeasible to apply in a realistic neural networks. In this section, we use greedy algorithms  reduce  complexity and improve running time of our framework.

 
\subsection{Gradient Coding} 


\subsection{Error Correction}




\subsection{Parallel Execution}

==> related.tex <==
\section{Related works}

==> setup.tex <==
\section{Experimental setup}
%\subsection{Implementation}
\label{sec:implementation}

We have implemented our algorithm in PyTorch~\cite{paszke2017automatic} and Tensorflow~\cite{tensorflow}. Unlike SGD, we need to compute the gradients per sample (or per $\mu-$batch), which makes it computationally expensive. We leverage multiple GPUs in parallel to speed up the training process. %We use Mathematica to compute the privacy bounds. 

%\red{everyone knows what MNIST and CIFAR are; We don't need to talk about their details}

We train models on MNIST and CIFAR10 datasets, with cross-entropy as the loss function.  We choose a training set up comparable to that of Abadi et al.~\cite{abadi2016deep}.\footnote{Available at~\url{https://github.com/tensorflow/privacy}} %In the case of MNIST, we choose our model's parameters similar to the latest model used by Abadi et al.~\cite{abadi2016deep}.\footnote{Available at~\url{https://github.com/tensorflow/privacy}} %What do you mean by choosing parameters? 



%\subsection{Datasets and Architectures}
%\paragraphb{MNIST}
%We use the MNIST image dataset which  consists of 70,000 instances of $28\times28$  handwritten grayscale digit images and the task is to recognize the digits. MNIST splits the training data to 60,000 images for training and 10,000 for the testing phase. We used a convolutional neural network with two convolutional layers and two fully connected layers for the MNIST experiments. 
%


%\paragraphb{SVHN}
% SVHN is a standard benchmark dataset which is consists of $32\times 32$ RGB images. The learning task is to classify the images into 10 classes of different objects. This dataset partitioned into 50,000 for training and 10,000 testing instances.
 
 
%\paragraphb{CIFAR}	We use CIFAR10, which  is a standard benchmark dataset consisting of $32\times 32$ RGB images. The learning task is to classify the images into 10 classes of different objects. This dataset is partitioned into 50,000 for training and 10,000 for testing. 
%We used the DenseNet~\cite{huang2017densely} model to train our classifier for these experiments.


%\paragraphb{Hyper-parameters} For both CIFAR10 and MNIST, we used cross-entropy as our loss function. 
%In case of MNIST, we chose our model's parameters similar to the latest model used by Abadi et al.~\cite{abadi2016deep}.\footnote{Available at~\url{https://github.com/tensorflow/privacy}} 



